Ultra Fast Deep Lane Detection with Hybrid Anchor Driven Ordinal Classification

Modern methods mainly regard lane detection as a problem of pixel-wise segmentation, which is struggling to address the problems of efficiency and challenging scenarios like severe occlusions and extreme lighting conditions. Inspired by human perception, the recognition of lanes under severe occlusions and extreme lighting conditions is mainly based on contextual and global information. Motivated by this observation, we propose a novel, simple, yet effective formulation aiming at ultra fast speed and the problem of challenging scenarios. Specifically, we treat the process of lane detection as an anchor-driven ordinal classification problem using global features. First, we represent lanes with sparse coordinates on a series of hybrid (row and column) anchors. With the help of the anchor-driven representation, we then reformulate the lane detection task as an ordinal classification problem to get the coordinates of lanes. Our method could significantly reduce the computational cost with the anchor-driven representation. Using the large receptive field property of the ordinal classification formulation, we could also handle challenging scenarios. Extensive experiments on four lane detection datasets show that our method could achieve state-of-the-art performance in terms of both speed and accuracy. A lightweight version could even achieve 300+ frames per second(FPS). Our code is at https://github.com/cfzd/Ultra-Fast-Lane-Detection-v2.

==> tables/aggregation.tex <==
\begin{table}[h]
	\centering
	\caption{Comparison between the four feature aggregation methods on the CULane dataset.}
	\setlength{\tabcolsep}{3.0mm}{
	\begin{tabular}{ccccc}
	\toprule
	Metric     & Avg & Max & Flatten & Flatten++ \\ \midrule
	F1-measure      & 67.76   & 55.83 & 74.46 & 74.00         \\ \bottomrule
	
    \end{tabular}}
	\label{tb_aggregation}
\end{table}


==> tables/aug.tex <==
\begin{table}[h]
    \centering
    \caption{Experiments of the data augmentation.}
    \label{tb_aug}
\begin{tabular}{lccc}
\toprule
Method     & mIoU  & Pixel Acc. & F1    \\
\midrule
ERFNet     & 61.2 & 95.9      & 73.1 \\
ERFNet+AUG &  61.1 & 95.9      & 73.1  \\
\bottomrule
\end{tabular}
\end{table}

==> tables/comparison_lstr.tex <==
\begin{table}[h]
    \centering
    \caption{The speed comparison between LSTR and UFLDv2.}
    \label{tb_lstr_speed}
    \begin{tabular}{lcccc}
    \toprule
    Settings & LSTR* & LSTR (360x640) & UFLDv2 (320x1600) & UFLDv2 (320x800)  \\ \midrule
    1-batched (FPS)    &  -   &  48 & 330 & 384 \\
    16-batched       &  420    & 675 & 480  & 928 \\
    
    \bottomrule
    \end{tabular}

    \medskip
    \emph{\footnotesize * means the reported speed from the original paper. All testings are conducted on an RTX 3090 GPU with CUDA 11.1 and PyTorch 1.8.2.} 
\end{table}

==> tables/culane_performance.tex <==
\begin{table*}[t]
    \caption{\red{Comparison of F1-measure and runtime on CULane testing set with IoU threshold=0.5. }}
	\vspace{-1em}
	\begin{tabular}{lccccccccccc}
		\toprule

		\textbf{Method} & \textbf{Normal} & \textbf{Crowded} & \textbf{Dazzle} & \textbf{Shadow} & \textbf{No line} & \textbf{Arrow} & \textbf{Curve} & \textbf{Crossroad} & \textbf{Night} & \textbf{FPS} & \textbf{Total} \\ \midrule

		SCNN~\cite{SCNN} & 90.6  & 69.7   & 58.5        & 66.9  & 43.4   & 84.1 & 64.4 & 1990   & 66.1 & 8                                     & 71.6 \\

		SAD~\cite{SAD} & 90.1  & 68.8   & 60.2        & 65.9  & 41.6   & 84.0 & 65.7 & 1998   & 66.0 & 75                                    & 70.8 \\

		ERFNet-IntRA-KD~\cite{hou2020interregion}   & - & - &   -   & -& - &  -      &     -   &   -     &   -     & 100                                    & 72.4 \\

		SIM-CycleGAN~\cite{SIM}    & 91.8  & 71.8   & 66.4        & 76.2  & 46.1   & 87.8 & 67.1 & 2346   & 69.4 &                -                      & 73.9 \\

		CurveLanes-NAS-S~\cite{xu2020curvelane}    & 88.3  & 68.6   & 63.2        & 68.0  & 47.9   & 82.5 & 66.0 & 2817   & 66.2 &            -                         & 71.4 \\

		CurveLanes-NAS-M~\cite{xu2020curvelane} & 90.2  & 70.5   & 65.9        & 69.3  & 48.8   & 85.7 & 67.5 & 2359   & 68.2 &               -                        & 73.5 \\

		CurveLanes-NAS-L~\cite{xu2020curvelane}  & 90.7  & 72.3   & 67.7        & 70.1  & 49.4   & 85.8 & 68.4 & 1746   & 68.9 &              -                      & 74.8 \\

		LaneATT (ResNet-18)~\cite{tabelini2021cvpr}    & 91.1  & 72.9   & 65.7        & 70.9  & 48.3   & 85.4 & 63.3 & 1170   & 68.9 & 250                                    & 75.1 \\

		LaneATT (ResNet-34)~\cite{tabelini2021cvpr}    & 92.1  & 75.0   & 66.4        & 78.1  & 49.3   & 88.3 & 67.7 & 1330   & 70.7 & 171            & 76.6 \\

		SGNet~\cite{su2021structure} & 91.4 & 74.0 & 66.8 & 72.1 & 50.1 & 87.1 & 67.0 & 1164 & 70.6 & 117  & 76.1 \\

		\midrule
		UFLD(ResNet-18) \cite{qin2020ultra}    & 87.7  & 66.0   & 58.4        & 62.8  & 40.2   & 81.0 & 57.9 & 1743   & 62.1 & 323                        & 68.4 \\

		UFLD(ResNet-34) \cite{qin2020ultra}   & 90.7  & 70.2   & 59.5        & 69.3  & 44.4   & 85.7 & 69.5 & 2037   & 66.7 & 175    & 72.3 \\      
		\midrule
		UFLDv2(ResNet-18)    & 91.7  & 73.0   & 64.6        & 74.7  & 47.2   & 87.6 & 68.7 & 1998   & 70.2 & 330                                   & 74.7  \\
		UFLDv2(ResNet-18)*    & 91.8  & 73.3   & 65.3        & 75.1  & 47.6   & 87.9 & 68.5 & 2075   & 70.7 & 310                                   & 75.0 \\

		UFLDv2(ResNet-34)    & 92.5  & 74.9   & 65.7        & 75.3  & 49.0   & 88.5 & 70.2 & 1864   & 70.6 & 165                                    & 75.9  \\
		UFLDv2(ResNet-34)*    & 92.5  & 74.8   & 65.5        & 75.5  & 49.2   & 88.8 & 70.1 & 1910   & 70.8 & 156                                    & 76.0 \\
		\bottomrule
		\end{tabular}
    
	\medskip
	\emph{For crossroads, only false positives are shown. The less, the better.
	`-' means the result is not available. \\
	* means our method with the feature level test time augmentation.}
	\label{tab:CULane compare}

\end{table*}


==> tables/curvelane.tex <==
\begin{table}[h]
    \centering
    \caption{Comparison on the CurveLanes dataset.}
    \label{tb_curvelane}
    \begin{tabular}{lcccc}
    \toprule
    Method       & F1    & Presicion & Recall & FPS \\ \midrule
    SCNN         & 65.02 & 76.13     & 56.74  & 8   \\
    SAD          & 50.31 & 63.60     & 41.60  & 75  \\
    PointLaneNet & 78.47 & 86.33     & 72.91  & 111 \\
    CurveLane-S  & 81.12 & 93.58     & 71.59  & \textless45  \\
    % CurveLane-M  & 81.80 & 93.49     & 72.71  &     \\
    % CurveLane-L  & 82.29 & 91.11     & 75.03  &    \\ 
    UFLDv2(ResNet-18)  & 80.45 & 81.49     & 79.44  &   145  \\ 
    UFLDv2(ResNet-34)  & 81.34 & 81.93     & 80.76  &   86  \\ 
    
    \bottomrule
    \end{tabular}
    \end{table}

==> tables/data_aug.tex <==
\begin{table}[h]
	\centering
	\caption{Comparasion between the models trained with and without data augmentations on the CULane Dataset.}
	\vspace{-1em}
	\begin{tabular}{cccc}
		\toprule
		Baseline & Data Augmentation & Training Acc & F1-measure \\ \midrule
		\checkmark &  & 24.83 & 37.68 \\
		\checkmark & \checkmark & 32.61 & 74.46 \\ \bottomrule
	\end{tabular}
\label{tab_data_aug}

\end{table}


==> tables/hyperparam_setting.tex <==
\begin{table}[]
    \centering
    \caption{Hyperparameter Settings on Different Datasets.}
    \vspace{-1em}
    \begingroup
    \setlength{\tabcolsep}{2mm}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{cc|cc}
    \toprule
      CULane &Value  & TuSimple & Value \\
    \midrule
                     $N_{row}$ & 18                      & $N_{row}$ & 56\\
                     $N_{col}$ & 40                      & $N_{col}$ & 40\\
                     $N_{dim}^r$ & 200                    & $N_{dim}^r$ & 100\\
                     $N_{dim}^c$ & 100                    & $N_{dim}^c$ & 100\\
                     $N_{lane}^r$ & 2                     & $N_{lane}^r$ & 2 \\
                     $N_{lane}^c$ & 2                      & $N_{lane}^c$ & 2 \\

    \bottomrule
    \end{tabular}
    \endgroup
    \label{tb_hyper}
\end{table}

==> tables/increase_row.tex <==
\begin{table}[h]
    \centering
    \caption{The performance of different number of row anchors.}
    \label{tb_increase_row}
    \begin{tabular}{lccccc|c}
    \toprule
    Number of row anchors & 18    & 36    & 72    & 144  & 288  & 144*  \\ 
    Spacing between anchors (pixels) & 17.8    & 8.9    & 4.4    & 2.2  & 1.1  & 2.2  \\ 
    \midrule
    F1-measure             & 66.09 & 67.60 & 68.77 & 69.38 & failed & 72.25 \\
    FPS                    & 341      & 331      &   301    &   259     &   -     &   259  \\
    \bottomrule
    \end{tabular}

    \medskip
    \emph{\footnotesize 144* means the post-processing strategy is specially tuned for the model with 144 row anchors, and it can be seen as the performance upper bound of the 144 row anchors setting. Details about post-processing strategy can be found in Q7 of Reviewer 2.} 
\end{table}

==> tables/tusimple.tex <==
\begin{table}[hbt]
    \centering
	\caption{Comparison with other methods on TuSimple test set. }
	\label{tab_tusimple}
	\begin{tabular}{lcccccc}
		\toprule
		Method   & F1 & Accuracy  & FP & FN & Runtime(ms) & Speed up \\ \midrule
		Res18-Seg & & 92.69 &&   & 25.3        &   5.3x       \\
		Res34-Seg  & & 92.84  &&  & 50.5        &   2.6x      \\
		LaneNet   & 94.80 & 96.38  & 7.80 &  2.44 & 19.0        &   7.0x      \\
		EL-GAN   & 96.26 & 94.90 & 4.12 &  3.36 & $>$100        &   $<$1.3x   \\
		SCNN    & 95.97 & 96.53  & 6.17 & 1.80 & 133.5       &   1.0x       \\
		SAD    & 95.92  & 96.64 & 6.02 &  2.05  & 13.4        &   10.0x     \\
	    FastDraw  & 93.92 & 95.20 & 7.60 & 5.40   & 11.1        &   12x     \\
	    LSTR & 96.85 & 96.18 & 2.91 & 3.38   & 20.8        &   6.3x     \\
		SGNet & & 95.87 && & 10.9 & 12.3x\\
		LaneATT (ResNet-18)  & 96.71 & 95.57 &3.56& 3.01 & 4.0 & 33.4x \\
		LaneATT (ResNet-34)  & 96.77 & 95.63 & 3.53 & 2.92 & 5.9 & 22.6x \\
		\midrule 
		\textit{protocol 1} \\
		UFLD(ResNet-18)     & 87.87 & 95.82  & 19.05 & 3.92 & 3.2         &   41.7x     \\ 
		UFLD(ResNet-34)     & 87.91 & 95.81   & 19.02 & 3.85 & 5.9        &   22.6x     \\
		UFLDv2(ResNet-18)   & 87.90 & 95.84 & 18.98 & 3.94  & 3.2         &   41.7x     \\ 
		UFLDv2(ResNet-34)   & 88.08 & 95.73 & 18.84 & 3.70  & 5.9         &   22.6x     \\ 
		\midrule
		
		\textit{protocol 2} \\
		UFLD(ResNet-18)     & 96.05 & 95.50  & 3.06 & 4.82 & 3.2         &   41.7x     \\ 
		UFLD(ResNet-34)   & 96.13 & 95.53 & 3.06 & 4.66  & 5.9         &   22.6x     \\ 
		UFLDv2(ResNet-18)   & 96.16 & 95.65 & 3.06 & 4.61  & 3.2         &   41.7x     \\ 
		UFLDv2(ResNet-34)   & 96.22 & 95.56 & 3.18 & 4.37  & 5.9         &   22.6x     \\ 
		\bottomrule
	\end{tabular}

\end{table}


==> tables/tusimple_performance.tex <==
\begin{table}[hbt]
	\caption{Comparison with other methods on TuSimple test set. }
	\label{tab:TuSimple compare}
	\vspace{-1em}
	\begin{tabular}{lccc}
		\toprule
		Method  & Accuracy & Runtime(ms) & Speed up \\ \midrule
		Res18-Seg \cite{chen2017deeplab}& 92.69    & 25.3        &   5.3x       \\
		Res34-Seg \cite{chen2017deeplab} & 92.84    & 50.5        &   2.6x      \\
		LaneNet \cite{End-to-End}  & 96.38    & 19.0        &   7.0x      \\
		EL-GAN \cite{ghafoorian2018gan}    & 96.39    & $>$100        &   $<$1.3x   \\
		SCNN \cite{SCNN}    & 96.53    & 133.5       &   1.0x       \\
		SAD \cite{SAD}      & 96.64    & 13.4        &   10.0x     \\
		SGNet~\cite{su2021structure} & 95.87 & 10.9 & 12.3x\\
		LaneATT (ResNet-18) \cite{tabelini2021cvpr} & 95.57 & 4.0 & 33.4x \\
		LaneATT (ResNet-34) \cite{tabelini2021cvpr} & 95.63 & 5.9 & 22.6x \\
		%	FastDraw  & 94.90    & 11.1        &   12x     \\
		\midrule 
		UFLD(ResNet-18)      & 95.87    & 3.2         &   41.7x     \\ 
		UFLD(ResNet-34)      & 96.06    & 5.9        &   22.6x     \\
		\midrule
		UFLDv2(ResNet-18)     & 96.03    & 3.2         &   41.7x     \\ 
		
		\bottomrule
	\end{tabular}

	\medskip
	\emph{\footnotesize The calculation of speed up is based on the slowest method SCNN. \\}
\end{table}


==> tex_files/exp.tex <==
\section{Experiments}
\label{sec_exp}
In this section, we demonstrate the effectiveness of our method with extensive experiments. The following sections mainly focus on three aspects: 1) Experimental settings. 2) Ablation studies of our method. 3) Results on two major lane detection datasets. 

\input{tables/exp_table.tex}

\subsection{Experimental setting}
\label{sec_setting}

\noindent
\textbf{Datasets.} To evaluate our approach, we conduct experiments on two widely used benchmark datasets: TuSimple Lane detection benchmark \cite{tusimple} and CULane dataset \cite{SCNN}. TuSimple dataset is collected with stable lighting conditions on highways. On the contrary, CULane dataset consists of nine different scenarios, including normal, crowd, curve, dazzle light, night, no line, shadow, and arrow in the urban area. The detailed information about the datasets can be seen in Table \ref{tab:dataset}.

\noindent
\textbf{Evaluation metrics.} The official evaluation metrics of the two datasets are different. For TuSimple dataset, the main evaluation metric is accuracy. The accuracy is calculated by: 
\begin{equation}
accuracy = \dfrac{\sum_{clip}C_{clip}}{\sum_{clip}S_{clip}} ,
\end{equation}
in which $C_{clip}$ is the number of lane points predicted correctly and $S_{clip}$ is the total number of ground truth in each clip.
As for the evaluation metric of CULane, each lane is treated as a 30-pixel-width line. Then the intersection-over-union (IoU) is computed between ground truth and predictions. Predictions with IoUs larger than 0.5 are considered as true positives. F1-measure is taken as the evaluation metric and formulated as follows:
\begin{equation}
F1-measure = \frac{2 \times Precision \times Recall}{Precision + Recall},
\end{equation}
where $Precision = \frac{TP}{TP + FP}$, $Recall = \frac{TP}{TP + FN}$ , $FP$ and $FN$ are the false positive and false negative.

\noindent
\textbf{Implementation details.} For both datasets, we use the row anchors that are defined by the dataset. Specifically, the row anchors of TuSimple dataset, in which the image height is 720, range from 160 to 710 with a step of 10. The counterpart of CULane dataset ranges from 260 to 530, with the same step as TuSimple. The image height of CULane dataset is 540. The number of gridding cells is set to 100 on the TuSimple dataset and 150 on the CULane dataset. The corresponding ablation study on the TuSimple dataset can be seen in \Cref{sec_ablation}. 

In the optimizing process, images are resized to 288$\times$800 following \cite{SCNN}. We use Adam \cite{kingma2014adam} to train our model with cosine decay learning rate strategy \cite{loshchilov2016sgdr} initialized with 4e-4. Loss coefficients $\lambda$, $\alpha$ and $\beta$ in Eq. 10 are all set to 1. The batch size is set to 32, and the total number of training epochs is set to 100 for TuSimple dataset and 50 for CULane dataset. The reason why we choose such a large number of epochs is that our structure-preserving data augmentation requires a long time of learning. The details of our data augmentation method are discussed in the next section. All models are trained and tested with pytorch \cite{paszke2017automatic} and nvidia RTX 2080Ti GPU. 

\noindent
\textbf{Data augmentation.}
Due to the inherent structure of lanes, a classification-based network could easily over-fit the training set and show poor performance on the validation set. To prevent this phenomenon and gain generalization ability, an augmentation method composed of rotation, vertical and horizontal shift is utilized. Besides, in order to preserve the lane structure, the lane is extended till the boundary of the image. The results of augmentation can be seen in Fig. \ref{fig_aug}.


\subsection{Ablation study}
\label{sec_ablation}
In this section, we verify our method with several ablation studies. The experiments are all conducted with the same settings as Sec. \ref{sec_setting}.

\noindent
\textbf{Effects of number of gridding cells.}
\label{ab_griding}
As described in Sec. 2, we use gridding and selecting to establish the relations between structural information in lanes and classification-based formulation. In this way, we further try our method with different numbers of gridding cells to demonstrate the effects on our method. We divide the image using 25, 50, 100 and 200 cells in columns. The results can be seen in Figure. \ref{fig_griding}. 
\begin{figure}[h]
	\centering
	\includegraphics[width=0.8\columnwidth]{figures/col_test.pdf}
	\caption{Performance under different numbers of gridding cells on the TuSimple Dataset. Evaluation accuracy means the evaluation metric proposed in the TuSimple benchmark, while classification accuracy is the standard accuracy. Top1, top2 and top3 accuracy are the metrics when the distance of prediction and ground truth is less than 1, 2 and 3, respectively. In this figure, top1 accuracy is equivalent to standard classification accuracy.}
	\label{fig_griding}
	\vspace{-10pt}
\end{figure}

With the increase of the number of gridding cells, we can see that both top1, top2 and top3 classification accuracy drops gradually. It is easy to understand because more gridding cells require finer-grained and harder classification. However, the evaluation accuracy is not strictly monotonic. Although a smaller number of gridding cells means higher classification accuracy, the localization error would be larger, since each gridding cell is too large to generate precise localization prediction. In this work, we choose 100 as our number of gridding cells on the TuSimple Dataset.



\noindent
\textbf{Effectiveness of localization methods.}
Since our method formulates the lane detection as a group classification problem, one natural question is what are the differences between classification and regression. In order to test in a regression manner, we replaced the group classification head in Fig. 5 with a similar regression head. We use four experimental settings, which are REG, REG Norm, CLS and CLS Exp. CLS means the classification-based method, while REG means the regression-based method. The difference between CLS and CLS Exp is that their localization methods are different, which are Eq. 2 and Eq. 3, respectively. The REG Norm setting is the variant of REG, which normalizes the learning target.

\begin{table}[h]
	\centering
	\caption{Comparison between classification and regression on the TuSimple dataset. REG and REG Norm are regression-based methods, while the ground truth scale of REG Norm is normalized. CLS means standard classification with the localization method in Eq. \ref{eq_argmax} and CLS Exp means the one with Eq. \ref{eq_approx}. }
	\setlength{\tabcolsep}{3.0mm}{
	\begin{tabular}{ccccc}
	\toprule
	Type     & REG & REG Norm & CLS & CLS Exp \\ \midrule
	Accuracy      & 71.59    &67.24 &95.77 & 95.87         \\ \bottomrule
	
    \end{tabular}}
	\label{tb_cls_reg}
\end{table}


The results can be seen in Table \ref{tb_cls_reg}. We can see that classification with the expectation could gain better performance than the standard method. This result also proves the analysis in Eq. \ref{eq_approx}. Meanwhile, classification-based methods could consistently outperform the regression-based methods. 




\noindent
\textbf{Effectiveness of the proposed modules.} In order to verify the effectiveness of the proposed modules, we conduct both qualitative and quantitative experiments. 

First, we show the quantitative results of our modules. As shown in Table \ref{tab:Module ablation}, the experiments are carried out with the same training settings and different module combinations. 



\begin{table}[h]
	\centering
	\caption{Experiments of the proposed modules on TuSimple benchmark with Resnet-34 backbone. Baseline stands for conventional segmentation formulation.}
	\label{tab:Module ablation}
    \setlength{\tabcolsep}{4mm}{
		\begin{tabular}{ccccc}
			\toprule
			Baseline & NF & SL & FA & Accuracy \\ \midrule
			\checkmark & & & & 92.84 \\
			 & \checkmark &  & & 95.64(+2.80)  \\
			 & \checkmark& \checkmark &  & 95.96(+3.12) \\
			 & \checkmark &  & \checkmark & 95.98(+3.14) \\
			 & \checkmark & \checkmark & \checkmark & 96.06(+3.22) \\ \bottomrule
	\end{tabular}}
\end{table}

From Table \ref{tab:Module ablation}, we can see that the new formulation gains significant performance improvement compared with segmentation formulation. Besides, both lane structural loss and feature aggregation could enhance the performance, which proves the effectiveness of the proposed modules. 

\begin{figure}[h]
	\centering
	\subfloat[W/O similarity loss]{\includegraphics[width=0.4\linewidth]{figures/col_test_new_1.png}}
    \hfil
	\subfloat[W/ similarity loss]{\includegraphics[width=0.4\linewidth]{figures/col_test_new_2.png}}
	\caption{Qualitative comparison of similarity loss. The predicted distributions of group classification of the same lane are shown. Fig. (a) shows the visualization of distribution without similarity loss, while Fig. (b) shows the counterpart with similarity loss.}
	\label{fig_col_test}
\end{figure}


Second, we illustrate the effectiveness of lane similarity loss in Eq. \ref{eq_sim}, the results can be seen in Fig. \ref{fig_col_test}. We can see that similarity loss makes the classification prediction smoother and thus gains better performance.

\subsection{Results}
In this section, we show the results on two lane detection datasets, which are the TuSimple lane detection benchmark and the CULane dataset. In these experiments, Resnet-18 and Resnet-34 \cite{resnet} are used as our backbone models.

For the TuSimple lane detection benchmark, seven methods are used for comparison, including Res18-Seg \cite{chen2017deeplab}, Res34-Seg \cite{chen2017deeplab}, LaneNet \cite{End-to-End}, EL-GAN \cite{ghafoorian2018gan}, SCNN \cite{SCNN} and SAD \cite{SAD}. Both TuSimple evaluation accuracy and runtime are compared in this experiment. The runtime of our method is recorded with the average time for 100 runs. The results are shown in Table \ref{tab:TuSimple compare}.


\begin{table}[h]
	\centering
	\caption{Comparison with other methods on TuSimple test set. The calculation of runtime multiple is based on the slowest method SCNN.}
	\label{tab:TuSimple compare}
	\begin{tabular}{lccc}
		\toprule
		Method  & Accuracy & Runtime(ms) & Multiple \\ \midrule
		Res18-Seg \cite{chen2017deeplab}& 92.69    & 25.3        &   5.3x       \\
		Res34-Seg \cite{chen2017deeplab} & 92.84    & 50.5        &   2.6x      \\
		LaneNet \cite{End-to-End}  & 96.38    & 19.0        &   7.0x      \\
		EL-GAN \cite{ghafoorian2018gan}    & 96.39    & $>$100        &   $<$1.3x   \\
		SCNN \cite{SCNN}    & 96.53    & 133.5       &   1.0x       \\
		SAD \cite{SAD}      & \textbf{96.64}    & 13.4        &   10.0x     \\
		%	FastDraw  & 94.90    & 11.1        &   12x     \\
		\midrule
		Res34-Ours      & 96.06    & 5.9        &   22.6x     \\ 
		Res18-Ours      & 95.87    & \textbf{3.2}         &   \textbf{41.7x}     \\ 
		
		\bottomrule
	\end{tabular}
\end{table}

From Table \ref{tab:TuSimple compare}, we can see that our method achieves comparable performance with state-of-the-art methods while our method could run extremely fast. The biggest runtime gap between our method and SCNN is that our method could infer 41.7 times faster. Even compared with the second-fastest network SAD, our method is still more than 2 times faster. 

Another interesting phenomenon we should notice is that our method gains both better performance and faster speed when the backbone network is the same as plain segmentation. This phenomenon shows that our method is better than the plain segmentation and verifies the effectiveness of our formulation.

For the CULane dataset, four methods, including Seg\cite{chen2017deeplab}, SCNN \cite{SCNN}, FastDraw \cite{FastDraw} and SAD \cite{SAD}, are used for comparison. F1-measure and runtime are compared. The runtime of our method is also recorded with the average time for 100 runs. The results can be seen in Table \ref{tab:CULane compare}. 
\begin{table*}[]
	\vspace{-5pt}
	\centering
	\caption{Comparison of F1-measure and runtime on CULane testing set with IoU threshold=0.5. For crossroad, only false positives are shown. The less, the better. `-' means the result is not available.}
	\label{tab:CULane compare}
	% \setlength{\tabcolsep}{0.4mm}{
		\begin{tabular}{lcccccccc}
			\toprule
			Category     & Res50-Seg\cite{chen2017deeplab} & SCNN\cite{SCNN}  & FD-50\cite{FastDraw} & Res34-SAD & SAD\cite{SAD}  & Res18-Ours & Res34-Ours \\ \midrule
			Normal       & 87.4      & 90.6  & 85.9     & 89.9    & 90.1   & 87.7    & \textbf{90.7}  \\
			Crowded      & 64.1      & 69.7  & 63.6     & 68.5    & 68.8   & 66.0& \textbf{70.2}  \\
			Night        & 60.6      & 66.1  & 57.8     & 64.6    & 66.0   & 62.1& \textbf{66.7}  \\
			No-line      & 38.1      & 43.4  & 40.6     & 42.2    & 41.6   & 40.2& \textbf{44.4}  \\
			Shadow       & 60.7      & 66.9  & 59.9     & 67.7    & 65.9   & 62.8& \textbf{69.3}  \\
			Arrow        & 79.0      & 84.1  & 79.4     & 83.8    & 84.0   & 81.0& \textbf{85.7}  \\
			Dazzlelight & 54.1      & 58.5  & 57.0     & 59.9    & \textbf{60.2}   & 58.4& 59.5  \\
			Curve        & 59.8      & 64.4  & 65.2     & 66.0    & 65.7   & 57.9& \textbf{69.5}  \\
			Crossroad    & 2505      & 1990  & 7013     & 1960    & 1998   & \textbf{1743}& 2037  \\ \midrule
			Total        & 66.7      & 71.6  &  -       & 70.7    & 70.8   & 68.4& \textbf{72.3}  \\ \midrule
			Runtime(ms)  &  -        & 133.5 &  -       & 50.5    & 13.4   & 3.1& 5.7   \\ 
			Multiple     &  -        & 1.0x  &  -       &  2.6x   &  10.0x & {43.0x}  & 23.4x \\   
			FPS          &  -        &  7.5  &  -       & 19.8    &  74.6  & {322.5} & 175.4 \\
			\bottomrule
	\end{tabular}
	% }
\end{table*}


It is observed in Table \ref{tab:CULane compare} that our method achieves the best performance  in terms of both accuracy and speed. It proves the effectiveness of the proposed formulation and structural loss on these challenging scenarios because our method could utilize global and structural information to address \textit{no-visual-clue} speed problem. The fastest model of our formulation achieves 322.5 FPS with a resolution of 288$\times$800, which is the same as other compared methods.

The visualizations of our method on the TuSimple lane detection benchmark and CULane dataset are shown in Fig. \ref{fig_vis}. We can see our method performs well under various conditions. %In some certain cases, like the results in the sixth row, the prediction is more straight and longer than the annotation. Moreover, the location of the leftmost lane is better than the annotation with bad lighting conditions and severe occlusion.

\begin{figure*}[t]

	\centering
	\includegraphics[width=0.9\linewidth]{figures/visall.pdf}
	\caption{Visualization on the TuSimple lane detection benchmark and the CULane dataset. The first four rows are results on the TuSimple dataset. The rest rows are results on the CULane dataset. From left to right, the results are image, prediction and ground truth, respectively. In the image, predicted lane points are marked in blue and ground truth annotations are marked in red. Because our classification-based formulation only predicts on the predefined row anchors, the scales of images and labels in the vertical direction are not identical.}
	\label{fig_vis}
\end{figure*}



==> tex_files/method.tex <==
\section{Method}
\label{sec_method}
In this section, we describe the details of our method. First, we demonstrate the definition of our formulation for lane detection. Second, based on the formulation, we show the network design of the backbone and classification head. Then, we illustrate the structural loss. At last, we elaborate on the set-based training pipeline.
\subsection{New formulation for lane detection}
\label{sec_formulation}
As described in the introduction section, fast speed and the no-visual-clue problems are important for lane detection. Hence, how to effectively handle these problems is key to good performance. In this section, we show the derivation of our formulation by tackling the speed and the no-visual-clue problem. For a better illustration, \Cref{tb_notation} shows some notations used hereinafter.
\input{tables/notation.tex}



\textbf{Definition of our formulation:} In order to cope with the problems above, we propose to formulate the problem of lane detection to a \textbf{row-based selecting method based on global image features}. In other words, our method is selecting the correct locations of lanes on each predefined row using the global feature. In our formulation, lanes are described as a series of horizontal locations at predefined rows, i.e., row anchors. In order to represent locations, the first step is gridding. On each row anchor, the location is divided into many cells. In this way, the detection of lanes can be described as selecting certain cells over predefined row anchors, as shown in Fig. \ref{fig_formulation_diff}(a). 

Suppose the maximum number of lanes is $N_l$, the number of row anchors is $N_r$, and the number of gridding cells is $N_c$. Suppose $X$ is the global image feature, and $f^{ij}$ is the classifier used for selecting the lane location on the $i$-th lane, $j$-th row anchor. Then the prediction of lanes can be written as:
\begin{equation}
	P_{i,j, :} = f^{ij}(X), \ \text{s.t.} \ \  i \in \{1,\cdots,N_l\}, j \in \{1,\cdots,N_r\},
	\label{eq_predict}
\end{equation}
in which $P_{i,j,:}$ is the $(N_c+1)$-dimensional vector represents the probability of selecting $(N_c+1)$ gridding cells for the $i$-th lane, $j$-th row anchor. Suppose $T_{i,j,:}$ is the one-hot label of correct locations. The generate of $T$ is shown in \Cref{fig_form}.  Then, the optimization of our formulation can be written as:
\begin{equation}
L_{cls}=\sum_{i=1}^{C} \sum_{j=1}^{h} L_{CE}(P_{i,j, :},T_{i,j, :}),
\end{equation}
in which $L_{CE}$ is the cross-entropy loss. The reason why our formulation is composed of $(N_c+1)$-dimensional classification instead of $N_c$-dimensional one is that an extra dimension is used to indicate the absence of lane.

From Eq. \ref{eq_predict} we can see that our method predicts the probability distribution of all locations on each row anchor based on global features, then the correct location can be selected based on the probability distribution.

\begin{figure*}[!t]
	\centering
	\subfloat[Our formulation]{\includegraphics[width=4.5in]{figures/form_diff1.pdf}%
    \label{fig_diff_our}}
    \hfil
	\subfloat[Segmentation]{\includegraphics[width=2.325in]{figures/form_diff2.pdf}%
    \label{fig_diff_seg}}
	\caption{Illustration of our formulation and conventional segmentation. Our formulation is selecting locations (grids) on rows, while segmentation is classifying every pixel. The dimensions used for classifying are also different, which is marked with red. The proposed formulation significantly reduces the computational cost. Besides, the proposed formulation uses global feature as input, which has a larger receptive field than segmentation, thus addressing the \textit{no-visual-clue} problem}
	\label{fig_formulation_diff}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/network_arch.pdf}
    \caption{Illustration of network architecture.}
    \label{fig_arch}
\end{figure*}

\textbf{How the formulation achieves fast speed:}
The differences between our formulation and segmentation are shown in Fig. \ref{fig_formulation_diff}. It can be seen that our formulation is much simpler than the commonly used segmentation. Suppose the image size is $H \times W$. In general, the number of predefined row anchors and gridding size is far less than the size of an image, that is to say, $N_r \ll H$ and $N_c \ll W$. In this way, the original segmentation formulation needs to conduct $H \times W$ classifications that are $N_l+1$-dimensional, while our formulation only needs to solve $N_l \times N_r$ classification problems that are $(N_c+1)$-dimensional. In this way, the scale of computation can be reduced considerably because the computational cost of our formulation is $N_l\times h\times (N_c+1)$ while the one for segmentation is $H\times W \times (N_l+1)$. For example, using the common settings of the CULane dataset \cite{SCNN}, the ideal computational cost of our method is $1.7\times10^4$ calculations, and the one for segmentation is $9.2\times 10^5$ calculations. The computational cost is significantly reduced, and our formulation could achieve extremely fast speed.

\textbf{How the formulation handles no-visual-clue problem:}
In order to handle the \textit{no-visual-clue} problem, utilizing information from other locations is important because \textit{no-visual-clue} means no information at the target location. For example, a lane is occluded by a car, but we could still locate the lane by information from other lanes, road shape, and even car direction. In this way, utilizing information from other locations is key to solve the \textit{no-visual-clue} problem, as shown in Fig. \ref{fig_difficult}.

From the perspective of the receptive field, our formulation has a receptive field of the whole image, which is much bigger than segmentation methods. The context information and messages from other locations of the image can be utilized to address the \textit{no-visual-clue} problem. 
From the perspective of learning, prior information like the shape and direction of lanes can also be learned using structural loss based on our formulation, as shown in Sec. \ref{sec_loss}. In this way, the \textit{no-visual-clue} problem can be handled in our formulation.
 
Another significant benefit is that this kind of formulation models lane location in a row-based fashion, which gives us the opportunity to establish the relations between different rows explicitly. The original semantic gap, which is caused by low-level pixel-wise modeling and high-level long line structure of lane, can be relieved.

\subsection{Network design}
\label{sec_net_design}

In this section, we show our network design with two parts, which are the backbone and classification head—the main goal of our network design to achieve fast speed while maintaining good performance. In this way, we use a latency-constrained neural architecture search method to get a high speed and performance backbone. Moreover, we use matrix factorization to reduce the large number of parameters and high computational cost in the classification head.
TODO
% \textbf{Backbone}
% % We use darts \cite{liu2019darts} as our search method. We use 
% Need to be revised.

% \textbf{classification head}
% As defined by the lane detection formulation in \Cref{sec_formulation}, we use classification based on global feature to directly learn the coordinates and locations of lanes. 


\subsection{Lane structural loss}
\label{sec_loss}


Besides the classification loss, we further propose two loss functions that aim at modeling location relations of lane points. In this way, the learning of structural information can be encouraged.

The first one is derived from the fact that lanes are continuous; that is to say, the lane points in adjacent row anchors should be close to each other. In our formulation, the location of the lane is presented by a classification vector. So the continuous property is realized by constraining the distribution of classification vectors over adjacent row anchors. In this way, the similarity loss function can be:
\begin{equation}
L_{sim}=\sum_{i=1}^{C} \sum_{j=1}^{h-1} \left \| P_{i,j,:} - P_{i,j+1,:} \right \|_1,
\label{eq_sim}
\end{equation}
in which $P_{i,j,:}$ is the prediction on the $j$-th row anchor and $\left \| \cdot \right \|_1$ represents L$_1$ norm.

Another structural loss function focuses on the shape of lanes. Generally speaking, most of the lanes are straight. Even for the curve lane, the majority of it is still straight due to the perspective effect. In this work, we use the second-order difference equation to constrain the shape of the lane, which is zero for the straight case.

To consider the shape, the location of the lane on each row anchor needs to be calculated. The intuitive idea is to obtain locations from the classification prediction by finding the maximum response peak. For any lane index $i$ and row anchor index $j$, the location $Loc_{i,j}$ can be represented as:
\begin{equation}
Loc_{i,j} = \argmax_k \, P_{i,j,k} \,, \  \text{s.t.} \ \   k \in \{1,2,\cdots,w\}  
\label{eq_argmax}
\end{equation}
in which $k$ is an integer representing the location index. It should be noted that we do not count in the background gridding cell and the location index $k$ only ranges from 1 to $N_c$, instead of $N_c+1$. 

However, the $\text{argmax}$ function is not differentiable and can not be used with further constraints. Besides, in the classification formulation, classes have no apparent order and are hard to set up relations between different row anchors. To solve this problem, we propose to use the expectation of predictions as an approximation of location. We use the softmax function to get the probability of different locations:
\begin{equation}
Prob_{i,j,:} = softmax(P_{i,j,1:w}),
\end{equation}
in which $P_{i,j,1:w}$ is a $N_c$-dimensional vector and $Prob_{i,j,:}$ represents the probability at each location. For the same reason as Eq. \ref{eq_argmax}, background gridding cell is not included and the calculation only ranges from 1 to $N_c$. Then, the expectation of locations can be written as: 

\begin{equation}
%loc \approx \sum_{j=1}^w prob_j \cdot j,
Loc_{i,j} = \sum_{k=1}^w k \cdot Prob_{i,j,k} 
\label{eq_approx}
\end{equation}
in which $Prob_{i,j,k}$ is the probability of the $i$-th lane, the $j$-th row anchor and the $k$-th location. The benefits of this localization method are twofold. The first one is that the expectation function is differentiable. The other benefit is that this operation recovers the continuous location with the discrete random variable.

According to Eq. \ref{eq_approx}, the second-order difference constraint can be written as:
\begin{equation}
\begin{split}
L_{shp} = \sum_{i=1}^C \sum_{j=1}^{h-2} & \| (Loc_{i,j} - Loc_{i,j+1}) \\
& - (Loc_{i,j+1} - Loc_{i,j+2}) \|_1,
\end{split}
\end{equation}
in which $Loc_{i,j}$ is the location on the $i$-th lane, the $j$-th row anchor.
The reason why we use second-order difference instead of first-order difference is that the first-order difference is not zero in most cases. So the network needs extra parameters to learn the distribution of first-order difference of lane location. Moreover, the constraint of second-order difference is relatively weaker than the one of first-order difference, thus resulting in less influence when the lane is not straight. Finally, the overall structural loss can be:
\begin{equation}
L_{str} = L_{sim} + \lambda L_{shp},
\label{eq_str}
\end{equation}
in which $\lambda$ is the loss coefficient.

\subsection{Feature aggregation}
\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/aggregation_new.pdf}
	\caption{Overall architecture. The auxiliary branch is shown in the upper part, which is only valid when training. The feature extractor is shown in the blue box. The classification-based prediction and auxiliary segmentation task are illustrated in the green and orange boxes, respectively. The group classification is conducted on each row anchor.}
	\label{fig_aggregation}

\end{figure*}

In Sec. \ref{sec_loss}, the loss design mainly focuses on the intra-relations of lanes. In this section, we propose an auxiliary feature aggregation method that focuses on the aggregation of the global context and local features. An auxiliary segmentation task utilizing multi-scale features is proposed to model local features. We use cross entropy as our auxiliary segmentation loss. In this way, the overall loss of our method can be written as:
\begin{equation}
L_{total} = L_{cls} + \alpha L_{str} + \beta L_{seg},
\label{eq_total}
\end{equation}
in which $L_{seg}$ is the segmentation loss, $\alpha$ and $\beta$ are loss coefficients.
The overall architecture can be seen in Fig. \ref{fig_aggregation}. 

It should be noted that our method only uses the auxiliary segmentation task in the training phase, and it would be removed in the testing phase. In this way, even we added the extra segmentation task, the running speed of our method would not be affected. It is the same as the network that doesn't utilize the auxiliary segmentation task.

==> tex_files/ref.tex <==
% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
\bibliography{egbibs}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)

    
    % biography section
    % 
    % If you have an EPS/PDF photo (graphicx package needed) extra braces are
    % needed around the contents of the optional argument to biography to prevent
    % the LaTeX parser from getting confused when it sees the complicated
    % \includegraphics command within an optional argument. (You could create
    % your own custom macro containing the \includegraphics command to make things
    % simpler here.)
    %\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
    % or if you just want to reserve a space for a photo:
    
    \begin{IEEEbiography}{Michael Shell}
    Biography text here.
    \end{IEEEbiography}
    
    % if you will not have a photo at all:
    \begin{IEEEbiographynophoto}{John Doe}
    Biography text here.
    \end{IEEEbiographynophoto}
    
    % insert where needed to balance the two columns on the last page with
    % biographies
    %\newpage
    
    \begin{IEEEbiographynophoto}{Jane Doe}
    Biography text here.
    \end{IEEEbiographynophoto}
    
    % You can push biographies down or up by placing
    % a \vfill before or after them. The appropriate
    % use of \vfill depends on what kind of text is
    % on the last page and whether or not the columns
    % are being equalized.
    
    %\vfill
    
    % Can be used to pull up biographies so that the bottom of the last one
    % is flush with the other column.
    %\enlargethispage{-5in}
    
    
    
    % that's all folks

==> tex_files/temlates_for_fig_table.tex <==
% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.
% However, the Computer Society has been known to put floats at the bottom.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that the IEEE does not put floats in the very first column
% - or typically anywhere on the first page for that matter. Also,
% in-text middle ("here") positioning is typically not used, but it
% is allowed and encouraged for Computer Society conferences (but
% not Computer Society journals). Most IEEE journals/conferences use
% top floats exclusively. 
% Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the
% \fnbelowfloat command of the stfloats package.

